Entropy-Based Decoding for Retrieval-Augmented Large Language Models

Augmenting Large Language Models (LLMs) with retrieved external knowledge has proven effective for improving the factual accuracy of generated responses. Despite their success, retrieval-augmented LLMs still face the distractibility issue, where the generated responses are negatively influenced by noise from both external and internal knowledge sources. In this paper, we introduce a novel, training-free decoding method guided by entropy considerations to mitigate this issue. Our approach utilizes entropy-based document-parallel ensemble decoding to prioritize low-entropy distributions from retrieved documents, thereby enhancing the extraction of relevant information of context. Additionally, it incorporates a contrastive decoding mechanism that contrasts the obtained low-entropy ensemble distribution with the high-entropy distribution derived from the model's internal knowledge across layers, which ensures a greater emphasis on reliable external information. Extensive experiments on open-domain question answering datasets demonstrate the superiority of our method.

==> tables/analyze_cad.tex <==
\begin{table}[!t]
    \renewcommand{\arraystretch}{1.05}
    \centering
    \small
    \begin{tabularx}{\linewidth}{l l XXX}
    \toprule
    Model &Method &NQ   &TQA    &WebQ  \\
    \midrule
    \multirow{2}{*}{\llama-2-7B}    &CAD &\textbf{38.92}  &65.92  &30.77 \\
            &\modelb~(Ours) &37.62     &\textbf{69.56}  &\textbf{36.12}  \\ 
    \midrule
    \multirow{2}{*}{\llama-2-13B}    &CAD &\textbf{39.43}  &68.96  &33.76 \\
            &\modelb~(Ours) &37.31     &\textbf{70.12}  &\textbf{38.19}  \\ 
    \midrule
    \multirow{2}{*}{Mistral-7B-v0.1}    &CAD &44.32  &70.27  &41.49 \\
            &\modelb~(Ours) &\textbf{46.32}     &\textbf{78.26}  &\textbf{49.76}  \\ 
    \midrule
    \multirow{2}{*}{\llama-3-8B}    &CAD &51.80  &79.01  &46.26 \\
            &\modelb~(Ours) &\textbf{52.02}     &\textbf{81.78}  &\textbf{51.62}  \\ 
    \bottomrule
    \end{tabularx}
    \vspace{-2mm}
    \caption{Performance under the top-5 document setting.}
    \vspace{-2mm}
    \label{tab:vanilla_cad}
\end{table}


==> tables/layer_selection.tex <==
\begin{table}[!t]
    \renewcommand{\arraystretch}{1.20}
    \centering
    \small
    \begin{tabularx}{\linewidth}{l p{1.75cm} XXX}
    \toprule
    Model &Baseline &NQ   &TQA    &WebQ  \\
    \midrule
    \multirow{4}{*}{LLAMA-2-7B}&w/o Contrast &25.48  &61.87  &20.25 \\
            &w/ FinalLayer &35.06     &62.89  &30.36  \\
             &w/ JSD       &35.07    &67.00   &32.19 \\
             &w/ Entropy    &\textbf{37.62}  &\textbf{69.56}  &\textbf{36.12} \\ 
    \midrule
    \multirow{4}{*}{LLAMA-2-13B}&w/o Contrast &36.54  &72.11  &34.63 \\
            &w/ FinalLayer &\textbf{38.59}    &\textbf{70.93}  &38.00  \\
             &w/ JSD       &18.12    &39.99   &15.50 \\
             &w/ Entropy    &37.62  &70.12  &38.19\\ 
    \midrule
    \multirow{4}{*}{LLAMA-3-8B}&w/o Contrast &51.74  &81.80  &52.17 \\
            &w/ FinalLayer &52.60    &81.36  &52.02  \\
             &w/ JSD       &51.83    &-   &51.38 \\
             &w/ Entropy    &51.58     &81.58  &51.67\\ 
    \bottomrule
    \end{tabularx}
    \caption{Different Layer Selection Strategy.}
    \label{tab:label_selection}
\end{table}
